A Dynamically Controlled Recurrent Neural Network for Modeling Dynamical Systems

This work proposes a novel neural network architecture, called the Dynamically Controlled Recurrent Neural Network (DCRNN), specifically designed to model dynamical systems that are governed by ordinary differential equations (ODEs). The current state vectors of these types of dynamical systems only depend on their state-space models, along with the respective inputs and initial conditions. Long Short-Term Memory (LSTM) networks, which have proven to be very effective for memory-based tasks, may fail to model physical processes as they tend to memorize, rather than learn how to capture the information on the underlying dynamics. The proposed DCRNN includes learnable skip-connections across previously hidden states, and introduces a regularization term in the loss function by relying on Lyapunov stability theory. The regularizer enables the placement of eigenvalues of the transfer function induced by the DCRNN to desired values, thereby acting as an internal controller for the hidden state trajectory. The results show that, for forecasting a chaotic dynamical system, the DCRNN outperforms the LSTM in $100$ out of $100$ randomized experiments by reducing the mean squared error of the LSTM's forecasting by $80.0\% \pm 3.0\%$.

==> old_proofs.tex <==

%We briefly reiterate the proof for the vanishing/exploding gradient problem with borrowed notations and assumptions from \cite{pascanu2013difficulty}:

%\begin{proof}
%First, we show the vanishing gradient case. Assume that $|\varphi^{'}(\cdot)|$ is bounded, and $\norm{diag(\varphi^{'}(\cdot))} \leq \gamma$. Let $\Lambda_{1}<\frac{1}{\gamma}$ be the largest singular value of the recurrent weight matrix $W_{rec}$. The Jacobian matrix $\frac{\partial h_{t+1}}{\partial h_{t}} = W^{T}_{rec}diag\big(\sigma^{'}(h_{t})\big)$. Then

%\begin{equation*}
%    \norm{\frac{\partial h_{t+1}}{\partial h_{t}}} 
%    \leq 
%    \norm{W^{T}_{rec}} \norm{diag\big(\varphi^{'}(h_{t})\big)} 
%    \leq 
%    \frac{1}{\gamma}\gamma < 1, 
%    \forall k. 
%\end{equation*}
%\\
%Let $\mathcal{E}_{t}$ be the error of the RNN at time $t$. Then it turns out that
%
%\begin{equation*}
%    \norm{\frac{\partial \mathcal{E}_{t}}{\partial h_{t}} \Bigg(\prod_{i=\tau}^{t-1} \frac{\partial h_{i+1}}{\partial h_{i}} \Bigg)} 
%    \leq 
%    \eta^{t-\tau} \norm{\frac{\partial \mathcal{E}_{t}}{\partial h_{t}}} 
%\end{equation*}
%\\
%Thus, for $\eta<1$ long-term contributions exponentially vanish over the interval between time-steps $t$ and $\tau$. The proof for exploding gradient follows by inverting the process above and for $\Lambda_{1} > \frac{1}{\gamma}$. 
%\end{proof}

%\begin{equation}
%    \frac{\partial E_{t}}{\partial h_{t}}
%    \cdot
%    \left[ \frac{\partial h_{t}}{\partial h_{t-1}}, \frac{\partial h_{t}}{\partial h_{t-2}}\right]
%    \cdot
%    \left[ \sum_{j=1}^{2}{\frac{\partial h_{t-1}}{\partial h_{t-1-j}}}; 
%    \sum_{j=1}^{2}{\frac{\partial h_{t-2}}{\partial h_{t-2-j}}}
%    \right]
%\end{equation}
